Isogeometric Boundary Elements in Electromagnetism: Rigorous Analysis, Fast Methods, and Examples

We present a new approach to three-dimensional electromagnetic scattering problems via fast isogeometric boundary element methods. Starting with an investigation of the theoretical setting around the electric field integral equation within the isogeometric framework, we show existence, uniqueness, and quasi-optimality of the isogeometric approach. For a fast and efficient computation, we then introduce and analyze an interpolation-based fast multipole method tailored to the isogeometric setting, which admits competitive algorithmic and complexity properties. This is followed by a series of numerical examples of industrial scope, together with a detailed presentation and interpretation of the results.

==> sec_maxwell.tex <==
%!TEX root = maxwell_siam.tex


Let $\Omega$ be compact with Lipschitz boundary, and if $\kappa > 0$ is a given positive wavenumber, we consider exterior scattering problems.
Given an incoming electric wave $\bb e_i$ satisfying the \emph{electric wave equation}
\begin{align}\label{eq:ewei}
\curl \curl \bb e_i -\kappa^2\bb e_i &= 0,
\end{align}
we are interested in calculating the wave $\bb e_s$ scattered by a perfectly
conducting scatterer $\Omega_s$, which is given by 
\begin{align}
\begin{aligned}
	\curl \curl \bb e_s -\kappa^2\bb e_s &= 0&&\text{in}~\overline{\Omega}:=\overline{\Omega_s}^c,\\
	\bb\gamma_t^+\bb e_s &= -\bb\gamma_t^+\bb e_i&&\text{on}~\Gamma:=\partial\Omega_s,
	\label{problem::ext_scattering}
\end{aligned}
\end{align}
together with the \emph{Silver-Müller radiation condition}. The total electric field
is then given by $\bb e = \bb e_i+\bb e_s$.

\begin{definition}
For $\bb w\in \bb H^{-1/2}_\times(\div_\Gamma,\Gamma)$, the \emph{electric
single layer potential} is given by
\begin{align}\label{eq:ESLP}
(\tilde{\MSL}_\kappa\bb w)(\bb x)
=
\int _\Gamma G_\kappa(\bb x-\bb y)\bb w(\bb y)\dd\sigma_{\bb y}
+
\frac{1}{\kappa^2}
\nabla_{\bb x}
\int _\Gamma G_\kappa(\bb x-\bb y)\div_{\Gamma}\bb w(\bb y)\dd\sigma_{\bb y}
\end{align}
for all $\bb x\notin\Gamma$, where $G_\kappa(\bb x-\bb y)$ is given by the
Helmholtz fundamental solution
\begin{align}\label{eq:HelmholtzGreen}
G_\kappa(\bb x-\bb y)=\frac{e^{-i\kappa\|\bb x-\bb y\|}}{4\pi\|\bb x-\bb y\|}.
\end{align}
\end{definition}
The electric single layer potential provides us with solutions to the
electric wave equation, see also \cite{Buffa_2003ab}.
\begin{lemma}
The electric single layer potential is a continuous operator
\[
\tilde{\MSL}_{\kappa}\colon \bb H^{-1/2}_\times(\div_\Gamma,\Gamma)\to\bb H_\loc(\bb\curl\,\bb\curl,\overline{\Omega}\cup\Omega_s)\cap\bb H_\loc(\div 0,\overline{\Omega}\cup\Omega_s).
\]
Moreover, for every $\bb w\in \bb H^{-1/2}_\times(\div_\Gamma,\Gamma)$,
$\tilde{\MSL}_\kappa\bb w$ is a solution to the electric wave equation
fulfilling the Silver-M\"uller radiation conditions.
\end{lemma}
Aiming at an indirect boundary element method, we make the ansatz
\[
\bb e_s=\tilde{\MSL}_\kappa\bb w\quad\text{in}~\overline{\Omega},
\]
and search for the unknown density $\bb w$, {which has a physical interpretation in terms of the \emph{surface current density}}.
. Taking the tangential trace on
both sides of the equation yields the \emph{electric field integral equation}
\begin{align}\label{eq:EFIE}
-\bb\gamma_t^+e_i=(\bb\gamma_t^+\tilde{\MSL}_\kappa)(\bb w)=:\MSL_\kappa\bb w.
\end{align}
\begin{lemma}
The \emph{electric single layer operator} $\MSL_\kappa:=\gamma_t^+\tilde{\MSL}_\kappa$ is a continuous mapping
$\MSL_\kappa\colon\bb H_\times^{-1/2}(\div_\Gamma,\Gamma)\to\bb H_\times^{-1/2}(\div_\Gamma,\Gamma)$
and, for non-resonant wavenumbers $\kappa$, invertible.
\end{lemma}


